Static Detection of DoS Vulnerabilities in Programs that use Regular Expressions (Extended Version)

In an algorithmic complexity attack, a malicious party takes advantage of the worst-case behavior of an algorithm to cause denial-of-service. A prominent algorithmic complexity attack is regular expression denial-of-service (ReDoS), in which the attacker exploits a vulnerable regular expression by providing a carefully-crafted input string that triggers worst-case behavior of the matching algorithm. This paper proposes a technique for automatically finding ReDoS vulnerabilities in programs. Specifically, our approach automatically identifies vulnerable regular expressions in the program and determines whether an "evil" input string can be matched against a vulnerable regular expression. We have implemented our proposed approach in a tool called REXPLOITER and found 41 exploitable security vulnerabilities in Java web applications.

==> analysis.tex <==
\newcommand{\fst}[1]{\emph{fst}(#1)}
\newcommand{\snd}[1]{\emph{snd}(#1)}

\section{Static Program Analysis}
\label{sec:analysis}

\todo{Shorten dramatically by describing it informally (or merging it with
  implementation section and making it ``system architecture'').}

\todo{Maybe move formal description to the appendix.}


So far, we have only focused on statically analyzing regular expressions, but as explained in Section~\ref{sec:overview}, the presence of a vulnerable regular expression does not necessarily mean that the program itself is vulnerable.  In this section, we describe  the program analysis component of our approach for determining if  the  program actually contains a vulnerability. At a high level, there are three questions we need to answer to determine whether  an application  contains a ReDoS vulnerability:

\begin{enumerate}
\item Is a variable $x$ that stores user input  matched against a vulnerable regular expression $\regex$?
\item Is it possible for $x$ to store an attack string for $\regex$?
\item Can the length of the string stored in $x$  exceed a minimum threshold
  specific to the matched regular expression $\regex$ that causes the matching algorithm to take significant time?~\footnote{If the length of $x$ cannot exceed a small constant $c$, then the running time of the matching algorithm will  also be bounded. The value of this constant $c$ depends on an input parameter to our algorithm and is computed using dynamic analysis of regular expressions (see Section~\ref{sec:impl}).}
\end{enumerate}

Clearly, the first question above can be easily answered using standard taint analysis. However, to answer the second question, we must employ a program abstraction that allows us to over-approximate the set of strings that can be stored in each program variable. Finally, to answer the third question, our program abstraction should also be capable of reasoning about lengths of strings.


To address these challenges,  we perform a static analysis that combines three different program abstractions, namely \emph{taint}, \emph{automata}, and \emph{intervals}.  Specifically, we employ the automaton abstraction to reason about string contents and use intervals to reason about string sizes.~\footnote{We are not the first ones to use automata for reasoning about string contents. For example, the {\sc Stranger}~\cite{Yu:2011,YuAlkhalaf2014} and {\sc Java String Analysis}~\cite{ChristensenMoller2003} tools also use automata for reasoning about string contents. We refer the reader to Section~\ref{sec:related} for a discussion of the similarities and differences.}





\begin{figure}
\[
\begin{array}{lll}
{\rm Statement} \ S & := & \ x := e \ | \ {\rm getInput}(x) \\
& & | \ {\rm match}(x, \regex) \ | \ S_1; S_2 \\
& & | \ {\rm assume}(x \in \impure) \\
& & | \ {\rm assume}(\len{x} \leq \nu)  \\
& & | \ {\rm if}(\star) \ {\rm then} \ S_1 \ {\rm else} \ S_2 \\
& & | \ {\rm while}(\star) \ {\rm do} \ S \\
& \\
{\rm String \ exp} \ e & := & x \ | \ ? \\
{\rm Int \ exp} \  \nu & := & {\rm int} \ | \ \len{x} \ | \ \nu_1 + \nu_2 \ | \ \nu_1 - \nu_2  \\  
{\rm Pure \ regex} \ \regex & := & a \in \Sigma \ | \  \regex^* \ | \ \regex_1 + \regex_2 \ | \ \regex_1 \cdot \regex_2 \\
{\rm Impure \ regex} \ \impure & := & \regex \ | \ x \ |  \  \impure^* \ | \ \impure_1 + \impure_2 \ | \ \impure_1 \cdot \impure_2 \\
\end{array}
\]
\vspace{-0.1in}
\caption{The \il intermediate language }
\vspace{-0.1in}
\label{fig:lang}
\end{figure}

\vspace{0.1in}
\noindent
{\bf \emph{Intermediate language.}} We describe our program analysis on the intermediate language shown in Fig.~\ref{fig:lang}. 
This language, which we refer to as \il, is suitable for describing our analysis because it  models the effects of different string manipulation functions in a uniform way using \emph{assume} statements. In Section~\ref{sec:impl}, we will explain how to convert Java programs into the intermediate language considered here.


In \il, all variables have type string. In addition to the standard  assignment, sequence, conditional, and loop constructs,  \il contains a  function  \emph{getInput(x)}, which binds variable $x$ to a string supplied by the user. Another  function, \emph{match($x, \regex$)},  models matching string $x$ against regular expression~$\regex$.  

The \il language contains two kinds of \emph{assume} statements that allow us to model the effect of string manipulation procedures (e.g., provided by {\tt java.lang.String}). First, the statement $\emph{assume}(x \in \impure)$ states that $x$ belongs to the language given by \emph{impure regular expression} $\impure$. Here, we refer to $\impure$ as \emph{impure} because the regular expression can refer to program variables. For example, the statement $\emph{assume}(x \in y \cdot a)$ models that the value stored in $x$ is the value stored in $y$ concatenated with the character $a$. Thus, if $y$ can be any string, then this annotation expresses that $x$ is a string ending in $a$. The use of such impure regular expressions in \il allows us to  model string operations in a uniform way.

The second form of annotation in \il is of the form $\emph{assume}(\emph{len}(x) \leq \nu)$ and allows us to express constraints on the size of strings. Here, the integer expression $\nu$ can refer to the length of other strings and can contain arithmetic operators ($+, -$).

One final point worth noting is that string expressions include a special symbol $?$, which represents an unknown string constant. Hence, an assignment of the form {\tt x = "abc"} is easily expressible in our language using the code snippet:
\[ x := ?;  \ {\rm assume}(x \in abc) \]


\begin{comment}
In order to describe our static analysis more precisely, we consider the simple language shown in Fig.~\ref{fig:lang}. In this language, we allow two kinds of expressions, namely variables, denoted $x$, and unknown string constants, denoted as $?$. Hence,  all expressions in this language have type string. In addition to assignments of the form $x:=e$, this language contains a function for querying user input. In particular, the statement ${\rm getInput(x)}$ queries the user for a string and stores the input in variable $x$. We also allow a special procedure, ${\rm match}$ that checks whether variable $x$ matches regular expression $\regex$. Hence, if $\regex$ is a vulnerable regular expression,  the statement ${\rm match}(x, \regex)$ corresponds to a sink. Our language also allows assume statements of the form ${\rm assume}(x \in \regex)$, which means that the value stored in variable $x$ belongs to the language of $\regex$. We use these assume statements to model sanitizers as well as concrete string constants. For instance, we can express the assignment $x := "abc"$ in our language using the code snippet:
\[ x := ?;  \ {\rm assume}(x \in abc) \]
Similarly, a function that removes all occurrences of character {\tt a} in a variable $x$ can be modeled using the assumption:
\[ {\rm assume} (x \in (\Sigma - {a} )^* ) \]
Finally, since our static analysis is path sensitive, we model predicates using $\star$, which represents  a non-deterministically chosen boolean value.
\end{comment}

\paragraph{Program abstraction.} As mentioned earlier, our program analysis needs to track taint information as well as information about string lengths and contents. Towards this goal, our analysis employs three kinds of program abstractions:
\begin{itemize}
\item The \emph{taint abstraction} $\Phi$ is a set of variables such that $x \in \Phi$ indicates that $x$ may be tainted.
\item The \emph{string abstraction} $\Lambda$ is a mapping from each program variable $x$ to a pair $(\interv, \automaton)$, where $\interv$ is an interval $\interval{l}{u}$ such that $l \leq \emph{len}(s) \leq u$ and $\automaton$ is an NFA representing $x$'s contents. In particular, if a string $s$ is in the language of $\automaton$, this indicates that $x$ can store string $s$.
\item The \emph{attack abstraction} $\Psi$ maps each regular expression $\regex$ in the program to a pair $(b, \attack)$. Here, $b$ is a minimum bound on the  length of the input string $s$ such that, if $\emph{len}(s) < b$, matching $s$ against $\regex$ takes negligible time~\footnote{Here, what constitutes \emph{negligible time} is an input parameter of our analysis and can be customized by the user. Furthermore,  the bound $b$ used in the attack abstraction is determined using dynamic analysis (see  Section~\ref{sec:impl}).}. The NFA $\attack$ is the attack automaton for regular expression $\regex$ and is pre-computed using the 
analyses from Sections~\ref{sec:regex} and ~\ref{sec:regex-superlinear}.
\end{itemize}

Since our program abstractions involve pairs (e.g., $(\interv, \automaton)$) , we use the notation \emph{fst(p)} and \emph{snd(p)} to retrieve the first and second components of pair $p$ respectively.


\begin{figure}
\[
\begin{array}{rll}
\evalregex{\regex}{\Lambda} & = & \automaton(\regex)  \\
\evalregex{x}{\Lambda} & = & \emph{snd}(\Lambda(x)) \\
\evalregex{\impure^*}{\Lambda} & = & (\evalregex{\impure}{\Lambda})^* \\
\evalregex{\impure_1 \impure_2}{\Lambda} & = & \evalregex{\impure_1}{\Lambda} \cdot \evalregex{\impure_2}{\Lambda} \\
\evalregex{\impure_1 + \impure_2}{\Lambda} & = & \evalregex{\impure_1}{\Lambda} + \evalregex{\impure_2}{\Lambda} \\
\end{array}
\]
\vspace{-0.1in}
\caption{Helper rules for evaluating impure regular expressions}\label{fig:eval-impure}
\vspace{-0.1in}
\end{figure}

\begin{figure}
\[
\begin{array}{rll}
\evalint{{\rm int}}{\Lambda} & = & \interval{{\rm int}}{{\rm int}}  \\
\evalint{\len{x}}{\Lambda} & = & \emph{fst}(\Lambda(x)) \\
\evalint{\nu_1 + \nu_2}{\Lambda} & = & \evalint{\nu_1}{\Lambda} \oplus  \evalint{\nu_2}{\Lambda} \\
\evalint{\nu_1 - \nu_2}{\Lambda} & = & \evalint{\nu_1}{\Lambda} \ominus  \evalint{\nu_2}{\Lambda} \\
\end{array}
\]
\vspace{-0.1in}
\caption{Helper rules for evaluating arithmetic expressions}\label{fig:eval-int}
\vspace{-0.1in}
\end{figure}

\begin{figure}
\[
\begin{array}{rll}
\interval{l_1}{u_1} \oplus \interval{l_2}{u_2} & = &  \interval{l_1+l_2}{u_1+u_2}  \\
\interval{l_1}{u_1} \ominus \interval{l_2}{u_2} & = &  \interval{l_1-l_2}{u_1-u_2}  \\
%\interval{l_1}{u_1} \sqcap \interval{l_2}{u_2} & = &  \interval{\emph{max}(l_1, l_2)}{\emph{min}(u_1, u_2)}  \\
\interval{l_1}{u_1} \sqcup \interval{l_2}{u_2} & = &  \interval{\emph{min}(l_1, l_2)}{\emph{max}(u_1, u_2)}  \\
(\Lambda_1 \sqcup \Lambda_2)(x) & = & (\fst{\Lambda_1(x)} \sqcup \fst{\Lambda_2(x)}, \\
& & \ \snd{\Lambda_1(x)} \cup \snd{\Lambda_2(x)})
\end{array}
\]
\vspace{-0.1in}
\caption{Operations on abstract domains}\label{fig:interval-ops}
\vspace{-0.1in}
\end{figure}

\paragraph{Analysis rules.} We describe our static analysis using judgments of the form
$
\Psi, \Phi, \Lambda \vdash S: \Phi', \Lambda'
$
which state that, if we execute $S$ in a state that satisfies program abstractions $\Psi, \Phi, \Lambda$, we obtain a new taint abstraction $\Phi'$ and new string abstraction $\Lambda'$. The inference rules describing our analysis are shown in Fig.~\ref{fig:rules}.




 
 \vspace{0.1in}


\begin{comment}
\begin{itemize}
\item $\Psi$, referred to as the \emph{attack environment}, maps each regular expression $\regex$ in the program to its corresponding \emph{attack automaton}. We assume that $\Psi$ has been generated using the regular expression analysis described in Section~\ref{sec:regex}.
\item $\Phi$, called the \emph{taint environment}, is a set that contains all {tainted} program variables. That is, $x \in \Phi$ indicates that $x$ may be under the control of the user. Note that $\Phi'$ represents the new taint environment obtained after analyzing statement $S$.
\item $\Lambda$, called the \emph{automaton abstraction},  maps each program variable $x$ to an automaton that accepts the strings that can be stored in $x$. Note that $\Lambda$ is an over-approximation: That is, if a string $s$ is not in the language accepted by $\Lambda(x)$, then $x$ cannot have value $s$, but not vice versa. Also, $\Lambda'$ represents the new automaton abstraction after analyzing statement $S$.
\end{itemize}
\end{comment}















\begin{figure}
\[
\begin{array}{cc}
(1) & \irule{
\begin{array}{c}
\Phi' = \Phi \cup \{ x \} \\
\Lambda' = \Lambda[x \mapsto (\interval{0}{\infty}, \automaton^*)]
\end{array}
}{
\Psi, \Phi, \Lambda \vdash {\rm getInput}(x): \Phi', \Lambda'
} \\ \ \\
(2) & \irule{
\begin{array}{c}
\Lambda' = \Lambda[x_1 \mapsto \Lambda(x_2)] \\
\Phi' = \left \{
\begin{array}{ll}
\Phi \cup \{x_1\} & {\rm if} \ x_2 \in \Phi \\
\Phi & {\rm if} \ x_2 \not \in \Phi
\end{array}
\right .
\\
\end{array}
}
{\Psi, \Phi, \Lambda \vdash x_1 := x_2: \Phi', \Lambda'}
\\ \ \\
(3) & \irule{
\Lambda' = \Lambda[x \mapsto (\interval{0}{\infty}, \automaton^*)]
}
{\Psi, \Phi, \Lambda \vdash x := \ ?: \Phi \setminus \{x\}, \Lambda'}  \\ \ \\
(4) & \irule{
\begin{array}{c}
\automaton = \emph{snd}(\Lambda(x)) \cap \evalregex{\impure}{\Lambda}\\
\Lambda' = \Lambda[x \mapsto (\emph{fst}(\Lambda(x)) , \automaton)]
\end{array}
}
{\Psi, \Phi, \Lambda \vdash {\rm assume}(x \in \impure): \Phi, \Lambda'}  \\ \ \\

(5) & \irule{
\begin{array}{c}
\interval{l_1}{u_1} =\emph{fst}(\Lambda(x))\\
\interval{l_2}{u_2} = \evalint{\nu}{\Lambda}\\
\interv = \interval{l_1}{\emph{min}(u_1, u_2)} \\
\Lambda' = \Lambda[x \mapsto ( \interv, \emph{snd}(\Lambda(x)))]
\end{array}
}
{\Psi, \Phi, \Lambda \vdash {\rm assume}(\len{x} \leq \nu): \Phi, \Lambda'}  \\ \ \\

(6) & \irule{
\begin{array}{c}
\automaton = \emph{snd}(\Psi(\regex)) \cap \emph{snd}({\Lambda(x)}) \\
x \not \in \Phi \lor \automaton = \automaton^\emptyset \lor \emph{fst}(\Psi(\regex)) \not \in \emph{fst}({\Lambda(x)})
\end{array}
}
{\Psi, \Phi, \Lambda \vdash {\rm match}(x, \regex): \Phi, \Lambda}  \\ \ \\
(7) & \irule{
\begin{array}{c}
\Psi, \Phi, \Lambda \vdash S_1: \Phi_1, \Lambda_1 \\
\Psi, \Phi_1, \Lambda_1 \vdash S_2: \Phi_2, \Lambda_2
\end{array}
}{\Psi, \Phi, \Lambda \vdash S_1; S_2: \Phi_2, \Lambda_2} \\ \ \\
(8) & \irule{
\begin{array}{c}
\Psi, \Phi, \Lambda \vdash S_1: \Phi_1, \Lambda_1 \\
\Psi, \Phi, \Lambda \vdash S_2: \Phi_2, \Lambda_2 \\
\Phi' = \Phi_1 \cup \Phi_2, \ \Lambda'= \Lambda_1 \sqcup \Lambda_2
\end{array}
}{\Psi, \Phi, \Lambda \vdash {\rm if}(\star) \ {\rm then} \ S_1 \ {\rm else} \ S_2:  \Phi', \Lambda' } \\ \ \\
(9) &
\irule{
\begin{array}{c}
\Phi^* \supseteq \Phi, \ \Lambda^* \sqsupseteq \Lambda \\
\Psi, \Phi^*, \Lambda^* \vdash S: \Phi^*, \Lambda^*
\end{array}
}
{\Psi, \Phi, \Lambda \vdash {\rm while}(\star) \ {\rm do} \ S: \Phi^*, \Lambda^*}
\end{array}
\]
\caption{Inference rules describing static analysis}
\label{fig:rules}
\end{figure}


In this figure, rule (1) describes the analysis of sources (i.e., $\emph{getInput}(x))$. Since variable $x$ is now tainted, we add it to our taint abstraction $\Phi$. Furthermore, since the user is free to supply any string,  $\Lambda'$ abstracts the length of $x$ using the interval $\interval{0}{\infty}$ and its contents using the automaton ~$\automaton^*$, which accepts any string.

Rule (2) for processing assignments $x_1 := x_2$ is straightforward: In particular, $x_1$ becomes tainted iff $x_2$ is tainted, and the string abstraction of $x_1$ is the same as variable $x_2$. For assignments of the form $x := ?$ (rule 3), we untaint variable $x$ by removing it from $\Phi$ since $?$ denotes string constants in \il. However, since $?$ represents unknown strings, $\Lambda'$ maps $x$ to $(\interval{0}{\infty}, \automaton^*)$.

Rule (4) describes the analysis of assumptions of the form $\emph{assume}(x \in \impure)$. Because $\impure$ can refer to program variables, we must first figure out the regular expressions that are represented by $\impure$. For this purpose, Fig.~\ref{fig:eval-impure} describes the evaluation of  impure regular expression $\impure$ under string abstraction $\Lambda$, denoted as $\evalregex{\impure}{\Lambda}$. Since the assumption states that the value stored in $x$ must be in the language $\evalregex{\impure}{\Lambda}$, the new string abstraction $\Lambda'$ maps $x$ to the automaton $\emph{snd}(\Lambda(x)) \cap \evalregex{\impure}{\Lambda}$.~\footnote{Observe that Rule (4) does not modify the length abstraction component of $\Lambda$. This is clearly sound, but potentially imprecise. However, since we model Java string operations by adding a pair of assumptions, one concerning length and the other concerning content, our analysis does not lead to a loss of precision because of the way assumptions are introduced.}

Rule (5), which is quite similar to rule (4), allows us to handle assumptions of the form $\emph{assume}(\emph{len}(x) \leq \nu)$. Since integer expression $\nu$ can refer to terms of the form $\emph{len}(y)$, we must evaluate $\nu$ under string abstraction $\Lambda$. For this purpose, Fig.~\ref{fig:eval-int} shows the evaluation of $\nu$ under $\Lambda$, denoted as $\evalint{\nu}{\Lambda}$. Now, going back to rule (5) of Fig.~\ref{fig:rules}, suppose that $\evalint{\nu}{\Lambda}$ yields the interval $\interval{l_2}{u_2}$, and suppose that $\Lambda$ maps $x$ to the length abstraction $\interval{l_1}{u_1}$. Clearly, the assumption $\emph{assume}(\emph{len}(x) \leq \nu)$ does not change the lower bound on $\emph{len}(x)$; hence the lower bound remains $l_1$. However, if $u_2$ is less than the previous upper bound $u_1$, we now have a more precise upper-bound $u_1$. Hence, the new string abstraction $\Lambda'$ maps the length component of $x$ to the interval $\interval{l_1}{\emph{min}(u_1, u_2)}$. 





Rule (6) for $\emph{match}$ statements allows us to detect if the program contains a vulnerability. In particular, 
the premise of this rule states that either (1) $x$ is \emph{not} tainted ($x \not \in \Phi$ ) or (2) the automaton representing $x$'s contents does not contain any string in the attack automaton for $\regex$ (i.e., $\automaton = \automaton^\emptyset$), or (3) the length of $x$ cannot exceed the minimum bound given by $\Psi$ (i.e., $\emph{fst}(\Psi(\regex)) \not \in \emph{fst}(\Lambda(x))$). If these conditions in the premise of the \emph{match} rule are not met, then the program may contain a vulnerability.


The next rules  for sequencing (7) and conditionals (8) are fairly standard. Since we take the union of the taint abstractions in rule (7),  a variable $x$ becomes tainted if it was tainted in either branch of the conditional. Also, note that the join operator on string abstractions is defined in Fig.~\ref{fig:interval-ops}.
Finally, the last rule describes the analysis of loops. In particular,  rule (9) states that the abstractions $\Phi^*$ and $\Lambda^*$ over-approximate the behavior of the loop because (a) they subsume the initial abstractions $\Phi, \Lambda$ (first premise), and (b) they are inductive (second premise). %Our implementation uses a very simple procedure to find loop invariants 
%Our implementation uses a simple guess-and-check procedure to find these loop invariants.

%While this rule does not describe how to compute $\Phi^*$ and $\Lambda^*$ in an algorithmic way, our implementation performs standard fixed point computation to find these loop invariants.
 
 \input{translation}
 
\begin{theorem}
\label{thm:soundness}
The analysis described in Fig.~\ref{fig:rules} is sound.
\end{theorem}

See Appendix A for a proof of Theorem~\ref{thm:soundness}.


% Local Variables:
% fill-column: 78
% TeX-master: "evil-regexes"
% End:


\begin{comment}
// old version before introducing numeric domain
\begin{figure}
\[
\begin{array}{cc}
(1) & \irule{
\begin{array}{c}
\Phi' = \Phi \cup \{ x \} \\
\Lambda' = \Lambda[x \mapsto \automaton^*]
\end{array}
}{
\Psi, \Phi, \Lambda \vdash {\rm getInput}(x): \Phi', \Lambda'
} \\ \ \\
(2) & \irule{
\begin{array}{c}
\Lambda' = \Lambda[x_1 \mapsto \Lambda(x_2)] \\
\Phi' = \left \{
\begin{array}{ll}
\Phi \cup \{x_1\} & {\rm if} \ x_2 \in \Phi \\
\Phi & {\rm if} \ x_2 \not \in \Phi
\end{array}
\right .
\\
\end{array}
}
{\Psi, \Phi, \Lambda \vdash x_1 := x_2: \Phi', \Lambda'}
\\ \ \\
(3) & \irule{
\Lambda' = \Lambda[x \mapsto \automaton^*]
}
{\Psi, \Phi, \Lambda \vdash x := \ ?: \Phi - \{x\}, \Lambda'}  \\ \ \\
(4) & \irule{
\Lambda' = \Lambda[x \mapsto (\Lambda(x) \cap \automaton(\regex))]
}
{\Psi, \Phi, \Lambda \vdash {\rm assume}(x \in \regex): \Lambda'}  \\ \ \\
(5) & \irule{
x \not \in \Phi \lor ((\Psi(\regex) \cap \Lambda(x)) = \automaton^\emptyset)
}
{\Psi, \Phi, \Lambda \vdash {\rm match}(x, \regex)} \\ \ \\
(6) & \irule{
\begin{array}{c}
\Psi, \Phi, \Lambda \vdash S_1: \Phi_1, \Lambda_1 \\
\Psi, \Phi_1, \Lambda_1 \vdash S_2: \Phi_2, \Lambda_2
\end{array}
}{\Psi, \Phi, \Lambda \vdash S_1; S_2: \Phi_2, \Lambda_2} \\ \ \\
(7) & \irule{
\begin{array}{c}
\Psi, \Phi, \Lambda \vdash S_1: \Phi_1, \Lambda_1 \\
\Psi, \Phi, \Lambda \vdash S_2: \Phi_2, \Lambda_2 \\
\Phi' = \Phi_1 \cup \Phi_2, \ \Lambda'= \Lambda_1 \sqcup \Lambda_2
\end{array}
}{\Psi, \Phi, \Lambda \vdash {\rm if}(\star) \ {\rm then} \ S_1 \ {\rm else} \ S_2:  \Phi', \Lambda' } \\ \ \\
(8) &
\irule{
\begin{array}{c}
\Phi^* \supseteq \Phi, \ \Lambda^* \sqsupseteq \Lambda \\
\Psi, \Phi^*, \Lambda^* \vdash S: \Phi^*, \Lambda^*
\end{array}
}
{\Psi, \Phi, \Lambda \vdash {\rm while}(\star) \ {\rm do} \ S: \Phi^*, \Lambda^*}
\end{array}
\]
\caption{Inference rules describing static analysis}
\label{fig:rules}
\end{figure}
\end{comment}


==> impl.tex <==



\section{Implementation}
\label{sec:impl}



We have implemented the ideas described in this paper in a new tool called \tool  for 
analyzing Java programs. The workflow of  \tool is shown in Fig.~\ref{fig:architecture} and
consists of the following main components:

\begin{comment}
Our approach consists of two main components: the regular expression analysis
for detecting (hyper-)vulnerable regular expressions (as described in
Sections~\ref{sec:regex} and \ref{subsec:regex-super-linear}) and the static
program analysis for checking if programs that make use of such vulnerable
regular expressions are unsafe (as described in
Section~\ref{sec:analysis}). In the following, we provide more details
about the implementation of each of these components.
\end{comment}

%\subsection{Regular Expression Analysis}

%The regular expression analysis itself makes use of two sub-components. 

\paragraph{Static RegEx Analysis.} This component implements the algorithms 
described in Sections~\ref{sec:regex} and~\ref{sec:regex-superlinear}. In
addition to specifying a regular expression, the user also specifies whether to detect
super-linear or exponential behavior. The output  is an attack automaton $\attack$
that captures all strings that trigger worst-case behavior.

Our implementation uses the {\sc Brics} library~\cite{brics} for converting regular expressions to NFA. However, since 
{\sc Brics} and Java regular expressions do not have the same syntax, our implementation first desugars Java regular expressions
into the {\sc Brics} format. If a Java regular expression $\regex$ uses features like backreferences that cannot be
expressed in {\sc Brics}, our current implementation fails to analyze $\regex$.





\todo{Mention that the dynamic analysis may introduce false negatives (see
  rebuttal).}

% From the rebuttal:
% Question 5: What are the limitations of the technique?
% Answer: While the approach is sound for the core language from Figure 12, there are features of the Java language that we do not analyze soundly (dynamic loading, reflection, etc). It is also true that the particular technique we use for finding a lower bound in the dynamic analysis may introduce false negatives. We will clarify this in our revision and explicitly discuss limitations.

\paragraph{Dynamic RegEx Analysis.} The goal of this component is 
 to determine the minimum number of repetitions of the attack core 
 that a given string must contain in order to trigger a specified time-out.
Given the original regular expression $\regex$, a specified time limit $t$, and the attack automaton $\attack$
(computed by previous analysis),  the dynamic component
produces a refined attack automaton as well as a number $k$ such that the length of the input string must exceed $k$
for the matching algorithm to take more than $t$ seconds.

In more detail, given an attack automaton $\automaton$ of the form $\automaton_p \cdot \automaton_c^+ \cdot \automaton_s$,
the dynamic analysis enumerates strings of the form $s_1 s^k s_2$ such that $s_1 \in \langu(\automaton_p)$, $s \in \langu(\automaton_c), s_2 \in \langu(\automaton_s)$ by repeatedly increasing the value $k$. In practice, this process does not require more than a few iterations because
we use the complexity of the NFA to predict the number of
repetitions that should be necessary based on previous runs. The smallest value of $k$ that causes the matching algorithm to exceed threshold $t$ is then used to compute the minimum required input length. This $k$ value is also used to refine the attack automaton: In particular, given the original attack automaton $\automaton_p \cdot \automaton_c^+ \cdot \automaton_s$, the dynamic analysis refines it to be $\automaton_p \cdot \automaton_c^k \cdot \automaton_c^* \cdot \automaton_s$. 


\paragraph{Program Analysis.} Unlike the previous analyses which operate on regular expressions, this component  analyzes Java source code. Specifically, given program $S$ and environment $\Psi$ (mapping regular expressions to attack automata), we use the analysis from Section~\ref{sec:analysis} to determine whether $S$ contains a vulnerability.  

Since the \il intermediate language used in Section~\ref{sec:analysis} contains assume statements, we must annotate methods in the Java string library in terms of the constructs supported by \il. While a full treatment of the {\tt java.lang.String} library is out of scope for this paper, Fig.~\ref{fig:translation} shows some representative examples that depict the correspondence between \il constructs and the Java string library. As shown in Table~\ref{fig:translation}, our translation is not fully precise: For instance, {\tt y = x.replaceAll(a, b)} is modeled using the assumption $\emph{assume}(y \in (!a)^*)$ and does not capture the fact that {\tt y} contains {\tt b} if {\tt x} contains {\tt a}. Our translation is deliberately not as precise as possible and tries to strike a good balance between minimizing false positives and keeping the analysis lightweight.

%\isil{Should we say something about how to compute loop invariants?}


\begin{comment}
\multicolumn{3}{ |c| }{Team sheet} \\
\hline
Goalkeeper & GK & Paul Robinson \\ \hline
\multirow{4}{*}{Defenders} & LB & Lucas Radebe \\
 & DC & Michael Duburry \\
 & DC & Dominic Matteo \\
 & RB & Didier Domi \\ \hline
\multirow{3}{*}{Midfielders} & MC & David Batty \\
 & MC & Eirik Bakke \\
 & MC & Jody Morris \\ \hline
Forward & FW & Jamie McMaster \\ \hline
\multirow{2}{*}{Strikers} & ST & Alan Smith \\
 & ST & Mark Viduka \\
\hline
\end{comment}


\begin{comment}

The dynamic analysis is run for each automaton ($\automaton_p \cdot
(\automaton_1 \cap \automaton_2)^+ \cdot \overline{\automaton_s}$ in the case
of hyper-vulnerable and $\automaton_p \cdot (\automaton_1 \cap \automaton_2
\cap \automaton_t)^+ \cdot \overline{\automaton_s}$ in the case of vulnerable
regular expressions) that was added to the attack automaton $\attack$ and that
actually recognizes some strings. The analysis determines how many repetitions
of the attack core are necessary to exceed the time limit chosen by the
user. This process runs attack strings with increasing number of
repetitions. In practice, this does not take more than a few iterations since
we use the complexity (exponential or super-linear) to predict the number of
repetitions that should be necessary based on previous runs. Once we determine
the number of repetitions $k$ we do not include attack strings with fewer
repetitions in the attack automaton $\attack_D$ that is produced by the
dynamic analysis.
\end{comment}



% Local Variables:
% fill-column: 78
% TeX-master: "evil-regexes"
% End:


==> soundness.tex <==
\section*{Appendix A: Soundness Proof (Theorem~\ref{thm:soundness})}
\label{sec:soundness}

\begin{proof} (sketch)
  To prove soundness we need to show that our abstract semantics
  over-approximates the concrete semantics of the language described in
  Fig.~\ref{fig:lang}. We will do so using the framework of abstract
  interpretation~\cite{cousot77}. The concrete state at a given point during
  the program execution is given by a function from variables to strings. Note
  that we will not consider taint here since our analysis follows the standard
  text book analysis for tracking explicit information flow using taint. Our
  abstract state captures the set of concrete states for each program point
  using a functional lifting of the Cartesian product of the automaton and
  the interval domain. In other words, our abstract state $\Lambda$ maps each variable
  to a tuple consisting of the automaton state and the interval state. Since
  this product construction is known to be sound~\cite{cousot77} we can prove
  the soundness of each abstraction individually.

  The interval domain~\cite{cousot77} is known to be sound and all rules from
  Fig.~\ref{fig:rules} modify the interval state, as expected, by
  over-approximating the concrete semantics of each statement: rules (1) and
  (3) set the state to top ($(0, \infty)$), rule (2) sets the state of the
  variable on the left-hand side to be the same as the state of the variable
  on the right-hand side, and rule (5) constrains the state of the variable
  $x$ to be less than or equal to the state of the expression $\nu$. The rules
  for the remaining statements, which may only reduce the set of possible
  concrete states,  do not modify the interval state, thus
  over-approximating it.

  The automaton domain makes use of the fact that regular languages form a
  lattice with $\automaton^{\emptyset}$ as the bottom element,
  $\automaton^{*}$ as the top element, and language inclusion as the partial
  order. Union and intersection act as join and meet, respectively. We can
  define an abstraction function $\alpha$ and a concretization function
  $\gamma$ to establish a Galois connection between the automaton domain and
  the the concrete domain of sets of strings. The function $\alpha$ turns each
  string into an automaton and forms their union, while the function $\gamma$
  enumerates all the accepting strings in the automaton. Given this, can show
  that all the statements over-approximate the concrete semantics according to
  our rules from Fig.~\ref{fig:rules}: rules (1) and (3) set the state to
  top ($\automaton^*$), rule (2) sets the state of the variable on the
  left-hand side to be the same as the state of the variable on the right-hand
  side, and rule (4) constrains the state of the variable $x$ to match the
  expression $\impure$, which amounts to forming the meet between the existing
  state and the state given by the expression $\impure$. The rules for the
  remaining statements, which may only reduce the set of possible concrete
  states, do not modify the automaton state and therefore over-approximate it.
\end{proof}

